Game-RL: Synthesizing Multimodal Verifiable Game Data to Boost VLMs' General Reasoning

Vision-language reinforcement learning (RL) has primarily focused on narrow domains (e.g. geometry or chart reasoning). This leaves broader training scenarios and resources underexplored, limiting the exploration and learning of Vision Language Models (VLMs) through RL. We find video games inherently provide rich visual elements and mechanics that are easy to verify. To fully use the multimodal and verifiable reward in video games, we propose Game-RL, constructing diverse game tasks for RL training to boost VLMs general reasoning ability. To obtain training data, we propose Code2Logic, a novel approach that adapts game code to synthesize game reasoning task data, thus obtaining the GameQA dataset of 30 games and 158 tasks with controllable difficulty gradation. Unexpectedly, RL training solely on GameQA enables multiple VLMs to achieve performance improvements across 7 diverse vision-language benchmarks, demonstrating the value of Game-RL for enhancing VLMs' general reasoning. Furthermore, this suggests that video games may serve as valuable scenarios and resources to boost general reasoning abilities. Our code, dataset and models are available at the GitHub repository.

==> sections/method.tex <==
\section{FR3E: First Return, Entropy-Eliciting Explore}
\label{sec:method}
Effective exploration in LLM reinforcement learning faces two primary obstacles: the loss of promising search trajectories and the inability to return to productive reasoning paths. Our approach, \textbf{FR3E}, addresses these challenges through a structured framework that explicitly separates the discovery of high-potential reasoning points from their systematic exploration.

The core idea is to decompose the reinforcement learning process into two complementary phases:
\begin{itemize}
    \item \textbf{First Return}: Identify key positions along base trajectories where model uncertainty is highest — potential forks in the reasoning space.
    \item \textbf{Entropy-Eliciting Explore}: From these identified states, perform diverse rollouts to sample alternative solution paths while maintaining semantic coherence.
\end{itemize}

This structured paradigm enhances traditional exploration-exploitation trade-offs by incorporating entropy-based signals directly into both path selection and policy update mechanisms.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.99\linewidth]{figure/main1.pdf}
    \caption{
Overview of the FR3E framework. \textbf{Stage 1: First Return} begins with base trajectory generation from query $q$, followed by token-wise entropy computation to identify high-uncertainty positions. These positions serve as segmentation points for constructing intermediate semantic states $S_j$. \textbf{Stage 2: Entropy-Eliciting Explore} launches multiple rollouts from each state $S_j$, evaluates the reward for each, and computes empirical values $V(S_j)$ to guide adaptive policy updates. This two-stage design encourages diverse yet structured exploration based on model uncertainty signals.
}

    \label{fig:main}
\end{figure}

\subsection{First Return: Block Definition via Uncertainty Signals}

\subsubsection{Base Trajectory Generation}

Given a training query $ q $, we first generate a base reasoning trajectory using the policy $ \pi_\theta $:
\begin{equation}
P_{\text{base}} = (q, t_1, t_2, \dots, t_L)
\end{equation}
where each $ t_i $ denotes a generated token in the response sequence. This trajectory represents the model's step-by-step reasoning process from the initial query to the final output.

\subsubsection{Entropy Computation}

To identify positions in the trajectory that exhibit high uncertainty — and thus are suitable for exploration — we compute the token-wise entropy at each position $ k $. Specifically, let:
\begin{equation}
\pi_\theta(v \mid q, t_{<k})
\end{equation}
denote the softmax-normalized probability distribution over the vocabulary at step $ k $, conditioned on the query $ q $ and previously generated tokens $ t_{<k} $.

We define the entropy of the policy at position $ k $ as:
\begin{equation}
H_k = -\sum_{v \in \mathcal{V}} \pi_\theta(v \mid q, t_{<k}) \log \pi_\theta(v \mid q, t_{<k})
\end{equation}
where $ \mathcal{V} $ is the model's vocabulary set.

Higher values of $ H_k $ indicate greater uncertainty in the model’s decision-making process at that position. These high-entropy positions represent promising candidates for initiating structured exploration.

\subsubsection{Entropy-Sensitive Position Selection}

Given the full base trajectory $ P_{\text{base}} $, we identify positions with maximal uncertainty by selecting the top-$ K $ tokens with highest entropy values. Specifically, we extract a set of entropy-sensitive positions:
\begin{equation}
\mathcal{K} = \{k_1, \dots, k_K\}
\end{equation}
which correspond to the most uncertain decision points along the reasoning path.

\textbf{Top-$ K $ Entropy Selection}: 
Select the indices corresponding to the $ K $ largest entropy values across the entire trajectory~\citep{wang20258020rulehighentropyminority}:
\begin{equation}
\mathcal{K} = \operatorname{TopK}\left( \{ H_k \}_{k=1}^L \right)
\end{equation}

This strategy ensures that we focus on the most uncertain reasoning steps globally, enabling us to identify natural forks in the model's reasoning space for structured exploration.

\newpage

\subsubsection{Semantic Block \& State Construction}

\begin{wrapfigure}{r}{0.5\textwidth}  % 'r' 表示右侧，宽度为50%
    \centering
    \vspace{-10pt}  % 可选，微调垂直位置
    \includegraphics[width=0.49\textwidth]{figure/high_entropy.pdf}
    \caption{Frequent tokens with the highest average entropy}
    \label{fig:high_entropy}
    \vspace{-10pt}  % 可选
\end{wrapfigure}
As shown in Figure~\ref{fig:high_entropy}, frequent tokens with high average entropy can be identified and used as key segmentation points. This figure is adapted from prior work~\citep{wang20258020rulehighentropyminority}, which analyzes token-level uncertainty across model trajectories. These entropy-sensitive positions serve as natural breakpoints for segmenting the trajectory into semantically meaningful reasoning blocks. Specifically, we define the block structure based on these key points:

\begin{equation}
P_{\text{base}} = B_1 \cup B_2 \cup \dots \cup B_{K+1}
\end{equation}
where each block $ B_n $ contains the subsequence of tokens between two consecutive entropy-sensitive positions:
\begin{equation}
B_n = (t_{k_{n-1}+1}, \dots, t_{k_n}), \quad \text{with } k_0 = 0, \; k_{K+1} = L
\end{equation}

From the previously identified entropy-sensitive positions $ \mathcal{K} $, we derive intermediate reasoning states:
\begin{equation}
S_j = (q, B_1, B_2, \dots, B_j)
\end{equation}
representing the full reasoning state up to and including block $ B_j $, just prior to the entropy-sensitive position $ k_j $.

This entropy-based segmentation provides structure for localized policy refinement and targeted credit propagation. It enables fine-grained control over which segments of the trajectory receive higher attention during optimization. By grounding exploration in model-intrinsic uncertainty signals, FR3E facilitates robust discovery of high-reward reasoning paths, particularly in tasks with sparse rewards and complex action spaces.

\subsection{Entropy-Eliciting Explore: Diversified Path Sampling from Anchors}

For each intermediate state $S_j$, we reset the context and generate $M$ diverse reasoning rollouts:
\begin{equation}
\mathcal{Y}_j := \{Y_{j,m}\}_{m=1}^M, \quad Y_{j,m} \sim \pi_\theta(\cdot \mid S_j)
\end{equation}

Each rollout $Y_{j,m}$ consists of a sequence of generated tokens extending from $S_j$. We define its reward based on whether the generated answer is correct:
\begin{equation}
r_{j,m} = 
\begin{cases}
1 & \text{if } Y_{j,m} \text{ is correct}, \\
0 & \text{otherwise}.
\end{cases}
\end{equation}

Using this reward definition, we estimate the empirical value of $S_j$~\citep{kazemnejad2024vineppounlockingrlpotential} as:
\begin{equation}
V(S_j) = \frac{1}{M} \sum_{m=1}^{M} r_{j,m}
\end{equation}

This value quantifies the average performance gain achieved when transitioning from the prefix $S_j$ to its extensions. It serves as a signal for adaptive policy updates during the Entropy-Eliciting Explore phase.

Through this mechanism, the model effectively samples from local neighborhoods around high-uncertainty prefixes, promoting diversity while preserving semantic coherence with the base trajectory. Specifically, by evaluating the correctness of each rollout, we can identify promising directions for exploration that are likely to lead to correct answers, thereby enhancing both the efficiency and effectiveness of the search process.


\subsection{Adaptive Advantage Modulation for Stable Learning}
\label{subsec:adaptive_advantage}

The phase of Entropy-Eliciting Explore generates a diverse set of rollouts from each intermediate state $S_j$, enabling precise estimation of the corresponding state values $V(S_j)$. To make effective use of this rich, structured reward signal for stable policy learning, we propose an adaptive mechanism that dynamically modulates the advantage function.

We introduce an advantage modulation factor, denoted $\alpha_j$, which scales the learning signal based on the marginal improvement in value from the previous state $S_{j-1}$ to the current state $S_j$:
\begin{equation}
\alpha_j = \frac{1}{\exp\left(V(S_j) - V(S_{j-1})\right)}.
\end{equation}
Using this factor, the modulated advantage $A'(S_j, P_{j,m})$ for a path $P_{j,m}$ originating at state $S_j$ is defined as:
\begin{equation}
A'(S_j, P_{j,m}) = \alpha_j \cdot A(S_j, P_{j,m}).
\end{equation}

The advantage modulation factor functions as a dynamic feedback controller during training. When $V(S_j) > V(S_{j-1})$, indicating a positive progression in reasoning quality, $\alpha_j < 1$. This reduces the influence of the advantage signal for successful paths, preventing premature convergence and preserving exploration diversity. Conversely, when $V(S_j) \leq V(S_{j-1})$, signaling stagnation or degradation in performance, $\alpha_j \geq 1$. This amplifies the learning signal, encouraging more aggressive exploration to overcome reasoning bottlenecks.

Under the idealized assumption that all trajectories within a block have identical length, the average of the modulated advantage across the entire batch is exactly zero:
\begin{equation}
\bar{A}' = \frac{1}{|\mathcal{T}|} \sum_j \alpha_j \sum_{(j, m) \in O_j} (r_{j, m} - V(S_j)) = 0,
\end{equation}
where $|\mathcal{T}|$ denotes the total number of tokens in the batch, and $V(S_j)$ is the empirical estimate of the value of state $S_j$.

Given that each trajectory in block $j$ contributes exactly $L_j$ tokens, the inner sum simplifies to:
\begin{equation}
\sum_{(j, m) \in O_j} (r_{j, m} - V(S_j)) = L_j \sum_{m=1}^{M} (r_{j, m} - V(S_j)),
\end{equation}
which equals zero by the definition of the empirical value. As a result, each term in the outer summation vanishes, leading to $\bar{A}' = 0$.

In practice, minor variations in trajectory lengths and other implementation details may cause deviations from this ideal condition. Nonetheless, the resulting policy gradient estimator remains approximately unbiased and theoretically grounded, while effectively incorporating the dense feedback obtained through structured exploration.
